Spatial-Temporal Residual Aggregation for High Resolution Video Inpainting

Recent learning-based inpainting algorithms have achieved compelling results for completing missing regions after removing undesired objects in videos. To maintain the temporal consistency among the frames, 3D spatial and temporal operations are often heavily used in the deep networks. However, these methods usually suffer from memory constraints and can only handle low resolution videos. We propose STRA-Net, a novel spatial-temporal residual aggregation framework for high resolution video inpainting. The key idea is to first learn and apply a spatial and temporal inpainting network on the downsampled low resolution videos. Then, we refine the low resolution results by aggregating the learned spatial and temporal image residuals (details) to the upsampled inpainted frames. Both the quantitative and qualitative evaluations show that we can produce more temporal-coherent and visually appealing results than the state-of-the-art methods on inpainting high resolution videos.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> introduction_backup.tex <==
\section{Introduction}
Video inpainting is a task of completing a given spatio-temporal region with newly synthesized contents. It has many applications , including video restoration \cite{chang2008application} , video editing (removing unwanted objects) \cite{abraham2012survey} \cite{bertalmio2001navier} , water mark removal \cite{lee2019copy} and video stabilization \cite{matsushita2006full} . There has been a growing number for deep learning methods which tries to solve this problem , but most of the methods cannnot perform well on high resolution videos due to lack of high resolution training data and also high memory requirements.
Before the advent of deep learning , most traditional methods used patch-based synthesis techniques \cite{huang2016temporally} \cite{newson2014video} \cite{wexler2007space}.These methods are often slow and have limited ability to synthesize new content and will require high memory usage to process high resolution videos. There are several groups of learning based methods which attempt to inpaint in a data driven manner. First group of methods used 3D convolution neural network with learn-able gated convolutions \cite{chang2019free} \cite{chang2019learnable} but due to memory contraints they can only apply their methods on low resolution short video sequences. Another group of methods learns the optical flow alignment to fill missing regions by aggregating information from nearby frames \cite{kim2019deep} \cite{xu2019deep} \cite{chang2019vornet} \cite{ding2019frame} \cite{koochari2010exemplar} . Some other methods tries to learn homograph based alignment  \cite{lee2019copy} \cite{woo2019align} and attention based alignment \cite{zeng2020learning} \cite{kim2019recurrent} \cite{oh2019onion}. Although promising results have been
shown, these methods have two major limitations that makes it hard to generalize well for high resolution videos . First limitation is due to high memory requirements for these methods thus these methods cannot run at their full potential for high resolution videos. Second limitations is the lack of availability of high resolution training data , so even these methods cannot generalise well at high resolution.
Inspired from \cite{yi2020contextual} , our target is to design a method that can be trained with low resolution videos but at inference can be used to process high resolution videos.On the core ideas behind video inpainting is that it inherently includes more cues for the problem as valid pixels for missing regions in a frame may
exist in other frames. As optical flow only provides a small temporal window to refer these contents and so may require large number of reference frames inorder to maintain temporal coherency , we choose a homograph based video inpainting technique \cite{lee2019copy} as our baseline and improves it algorithm . We propose an end to end DNN based video painting network with 3 stages : First stage is a self supervised homograph based alignment network similar to \cite{lee2019copy} , Second stage takes in the aligned frames and learns a attention map to copy features at multiple resolutions using skip connections and the third stage does image inpainting on the regions where no reference features are found using a network inspired from \cite{yi2020contextual}.All the three stages are trained end to end . Image residuals are  difference between an image and the blurred version of itself . This concept is employed to decompose every frame of the video into low frequency and high frequency images. At inference time , the network takes in this low frequency images to output the result at low resolution and is up sampled to the original resolution and the residual post processing unit improves the final result by adding the residuals using the learned temporal and spatial attention map .
In summary the major contribution of our paper is as follows:
\begin{itemize}
	\item A residual unit which uses the learnt alignments matrices , temporal and spatial attention maps from the network to transfer the inpainted region to high resolution .The model can
	be trained on small images and applied on large images, which significantly alleviates the requirements
	for high-resolution training datasets.
	\item A novel temporal aggregation network which learns a temporal attention map at low resolution and Transfers them to other layers to recover high frequency information from the reference frames. This attention is also used to compute a temporal left-over mask where no reference features were found and also provides a good first estimate for the region using dilated convolutions .
	\item A spatial aggregation network inspired from \cite{yi2020contextual} , which takes in the output from the temporal aggregation network and the temporal left-over mask to futher refine the results by using contextual attention transfer .
	\item Use homography and optical flow alignments to combine long range sparse correspondaces and short range dense correspondences and combine them use temporal context aggregation.
	\item Improve temporal contextual aggregation quality by adding scaled softmax and multiscale feature aggregation.
	\item A synthetic test video inpainting dataset to do quantitative evaluation 
	  
\end{itemize}    


==> method_backup.tex <==
\section{Method}

\begin{figure*}
	\includegraphics[width=\linewidth]{overview.png}
	\caption{Spatio-Temporal Residual post processing to transfer the low resolution result to the original input resolution to be used at inference}
	\label{fig:overview}
\end{figure*}  


%\begin{figure}
%	\includegraphics[width=\columnwidth ,scale=0.5]{temporal_aggregagation.jpg}
%	\caption{Temporal Aggregation Branch}
%	\label{fig:t_agg}
%\end{figure}

\subsection{Overview}
The overview of our spatial-temporal aggregation (STA) network is shown in Figure \ref{fig:overview}. The
system takes a video (X) annotated with the missing pixels (M) in each frame and outputs the completed video (Y). All the raw frames (X) and masks (M) are padded and down-sampled to 512x512 resolution. Down-sampled frames (x) and masks (m) are up-sampled to their raw resolution and subtracted from raw frames to get the residuals (R). The video is processed frame-by-frame in the temporal order. We refer the frame to be filled as the target frame and the other frames as the reference frames. The temporally far away reference frames are aligned to the target frames using a global affine transformation and nearby frames are aligned using optical flow. The aligned reference frames and masks along with the target frames and masks are processed by the temporal aggregation network which decides which pixels to copy from which reference frames and also outputs a temporal left-over mask ($m^{t1}$) which constitutes the region where no reference pixels were found. The temporally completed image ($y^{t1}$) along with the temporal left-over mask ($y^{t1}$) is processed by the spatial aggregation network which searches for contextual patches in the target frame and fills the left-over region($y^{t2}$). In the end, the residual aggregation module uses the learned alignment matrices, temporal and spatial attention maps from the network to generate a sharp inpainted frame in the original resolution $Y^{t}$. The inpainted frame will subsequently be used as a reference frame, providing more information for filling the following frames. 
   	
\subsection{Copy-Paste Summary}
Copy-Paste Network \cite{lee2019copy} is a 2-stage network where the first stage computes affine transformation to align the reference frames to the target frame and the second stage computes the features that can be copied from the aligned reference frames using a context matching module to complete and reconstruct the target frame. The Alignment Network is trained by minimizing the pixel wise L1 distance between target frame and the aligned reference frame on the regions where the pixels are valid in both the frames.

The second stage maps the aligned frames and target frame to a low resolution feature space. The context matching module computes cosine similarities ($T_{a,b}$) between the target and reference feature maps $F^a (x, y)$ and $F^{b}(x, y)$ weighted by their corresponding masks $m^a$ and $m^b$ as in the bottleneck as follows:
\begin{equation} \label{eq:1}
V(x,y) = m^a \cdot m^{b}
\end{equation}
\begin{equation} \label{eq:2}
T_{a,b} = \frac{1}{\sum_{(x,y)} V(x,y)} \cdot \sum_{(x,y)} V(x,y) \cdot F^a (x, y) \cdot F^{b}(x, y)
\end{equation} 
\begin{equation} \label{eq:att}
S_{a,b} = softmax(T_{a,b} \cdot V_{a, b})
\end{equation} 
where $a$ is target feature map and $b$ is a set of reference feature maps. The cosine similarity $T_{a,b}$ for each target-reference pair is multiplied with its corresponding visibility map V(x,y) \ref{eq:1}. Then a masked softmax \ref{eq:att} is applied on the valid regions to compute the weight of each pixel as the attention score in the reference frame set to reconstruct and inpaint the target frame. Note that in \eqref{eq:att}, $V_{a, b}$ refers to the visibility map of the reference aligned to the
target. Next, the reference features and masks are aggregated using the computed attention scores and concatenated with the target features and fed to a decoder, which consists of several dilated convolution blocks and up-sampling modules. The decoder recovers the target frame by filling the holes with reference features when available and generates the pixels using dilated convolutions when reference information is not available .  

\begin{figure*}
	\includegraphics[width=\textwidth]{arch.png}
	
	\caption{Overview of the STA-network}
	\label{fig:sta-net}
\end{figure*}

\subsection{Global/Local Alignment Network}
For robust video inpainting , find the best temporal window is crucial to copy valuable and relevant contents from the other frames. Global affine transformation based alignment \cite{lee2019copy} is best suited for static background and provides a large temporal window to copy information from distant frames. With optical flow based alignment \cite{xu2019deep}, the temporal range of information is small but it can handle dynamic motion in the background and therefore provide local dense pixel alignment. In our approach, we added the pre-trained PWC-IRR network \cite{hur2019iterative} as an additional alignment branch to achieve the benefits from both global and local alignment. In the ablation studies, we show that the proposed global/local alignment network achieves the best results both quantitatively and qualitatively.

\subsection{Multi-Scale Temporal Aggregation Network}
After the image alignment, the aligned images are converted into multi-scale feature maps by using a shared encoder. 
The cosine similarity scores are calculated using the feature maps at lowest resolution as shown in Equations (\ref{eq:1}) and (\ref{eq:2}), and the attention scores are calculated between the target features and all reference features using Equation (\ref{eq:att}). This ensures selective fusion of reference features when generating the missing features in target frames.

\paragraph{Multi-scale temporal attention transfer.} To more efficiently utilize the context matching information between the target frame and the reference frames, the cosine similarity scores $T_{a,b}$ computed in Equation (\ref{eq:2}) are shared multiple times as shown in Figure \ref{fig:sta-net} by resizing the masks $m^a$ and $m^b$ at each level. The attention score $S_{a,b}$ is then calculated for each level and we show that the proposed multi-scale temporal aggregation module achieves much better results compared to the vanilla temporal aggregation network in the original Copy-Paste Network in our experiment analysis.
%\subsection{Temporal Aggregation Network}
%
%After the frame alignment , the aligned frames are converted into multi-resolution features by using a shared encoder .The temporal matching module computes a attention map using the features at lowest resolution indicating the importance of each feature in the encoding frame to recover the target frame by the filling in the missing information from the residual features. The temporal attention transfer module is used to apply the calculated attention to each resolution using skip connections from encoder to decoder and also calculates a temporal left-over mask where no reference features were found . The decoder recovers the completed target frame with contents transferred using the attention module and also a good first estimate for the temporal left-over region .
%
%\textbf{Copy Encoder} Encoder network consists of a series of convolution block which takes the input RGB image and corresponding binary masks and outputs a multi-scale feature maps as shown in fig \ref{fig:t_agg}
%
%\textbf{Temporal Attention Computation} temporal attention is calculated as cosine similarities ($T_{a,b}$) between the 2 features map $F^a (x, y)$ and $F^{b}(x, y)$ weighted by their corresponding masks $m^a$ and $m^b$ as in the bottleneck as follows:
%\begin{equation} \label{eq:1}
%V(x,y) = m^a \cdot m^{b}
%\end{equation}
%\begin{equation} \label{eq:2}
% T_{a,b} = \frac{1}{\sum_{(x,y)} V(x,y)} \cdot \sum_{(x,y)} V(x,y) \cdot F^a (x, y) \cdot F^{b}(x, y)
%\end{equation}
%where $a$ is target feature map and $b$ is a list of target and reference features maps as shown in \ref{fig:t_agg} and the values are stored as a list which will be used by Multi-scale Temporal Attention Transfer module .The self cosine similarity of target features are also calculated. This ensures seamless fusion of required feature when the information from target feature maps and reference maps to the decoder.
%
%\textbf{Multi-scale Temporal Attention Transfer} Using the temporal attention values $T_{a,b}$ computed in Eqn  \ref{eq:2} , this module fuses the target and reference feature maps from encoder using masked softmax from \cite{lee2019copy}. The $T_{a,b}$ scores are shared multiple times as shown in Fig.\ref{fig:t_agg} by resizing the masks $m^a$ and $m^b$ at each level. This leads to improvement in quality and also fewer parameters and better efficiency in terms of memory and speed. 
%
%\textbf{Decoder} The multi scale aggregated features from target and reference frames are fed into the decoder which consists of series of convolution and up-sampling modules and recovers the target frame by filling the holes with reference features when available and generates the pixels using dilated convolutions when reference information is not available .

\subsection{Spatial Aggregation Network}
Although the temporal aggregation network already provides an initial estimate for the temporal left-over region ($Y^{t1}$), it often has visual artifacts. To further improve the inpainting quality, the left-over mask ($M^{t1}$).$Y^{t1}_{out}$ is blended with the $X^{t}$ using $M^{t1}_{out}$ as input to a spatial aggregation network ($F_s$) which has similar architecture as the refine network in \cite{yi2020contextual}. This spatial aggregation network calculates contextual attention scores at the lowest resolution feature map and performs attention transfer on multiple higher resolution feature maps to improve the quality of final inpainted region for hole regions that cannot be filled from all reference frames. The network also outputs a spatial attention score ($S_{i,j}$) which is a similarity score between $i^{th}$ patch from context with $j^{th}$ patch from the hole. This spatial attention score will be used in the proposed residual aggregation module to further improve the image quality.
 \begin{equation} \label{eq:3}
 y^{t1}_{in} = y^{t1}_{out} * (1 - m^{t1}) + x^{t} * (m^{t1})
 \end{equation}
 \begin{equation} \label{eq:4}
 y^{t2} , S_{i,j} =F_s( y^{t1}_{in} , m^{t1} )
 \end{equation}



\subsection{Temporal/Spatial Residual Aggregation}
The spatial-temporal aggregation network generates inpainted image in low-resolution, mainly due to the memory constraints. To generate the inpainted image in the original resolution, one can naively up-sampled the output. However, this process normally generate blurry results. Inspired by the contextual residual aggregation algorithm in \cite{yi2020contextual}, we applied the contextual residual aggregation process using both temporal and spatial attention scores, which are calculated by temporal and spatial aggregation networks described above. This entire process is demonstrated in Figure ~\ref{fig:overview}. The temporal attention scores are used to transfer the high-frequency details from reference frames to the current frame, for the missing regions that are temporal available. On the other hand, the spatial attention scores are used to transfer the high-frequency details from surrounding patches to the missing patch in the current frame. By adding these contextual transferred high-frequency details, we succeed to generate sharp inpainted output ($Y^{t2}$) at its original resolution.

%\begin{algorithm}
%	\small
%	\caption{Inference and Residual Post-processing}
%	\label{alg:inference}
%	\SetAlgoLined
%	Input: Raw frame $X^t$ with mask $M^t$ ($t = 0,1,...,n$) \\	
%	Input: Downsampled frame $x^t$ (bilinear) with mask $m^t$ (nearest) ($t = 0,1,...,n$) \\
%	Input: Upsample $x^t$ and substract from  $X^t$ to calcualte residuals $R^t$ ($t = 0,1,...,n$)\\
%	Input: Number of reference frame for $N_{ref}$\\
%	Output: Inpainted frame $Y^{t2}$ ($t = 0,1,...,n$) \\
%	\For{t = 1,2,...,T-1}{
%		calcuated indices for refernce frame $i_{ref}$ = ($t-N_{ref}$,...,$t+N_{ref}$) \\
%		Multi-scale Target Copy features $F^t$ = Copy Encoder($x^t$,$m^t$) \\
%		\For{r in $i_{ref}$}{
%			\If{r is t-1 or t-2 }{ 
%				Flow $F^r_{trans}$ = PWC-IRR ($x^t$,$x^r$) \\
%				$x^{r\rightarrow t}$ ,$m^{r\rightarrow t}$ = Warp ($x^r$,$m^t$,$F^r_{trans}$) \\
%			}
%			\Else{
%				Affine Transformation $A^r_{trans}$ = Alignment Network($x^t$,$m^t$ ,$x^r$,$m^t$) \\
%				$x^{r\rightarrow t}$ ,$m^{r\rightarrow t}$ = Warp ($x^r$,$m^t$,$A^r_{trans}$) \\
%			}
%		
%			
%			Multi-scale Reference Copy features $F^r\rightarrow t$ = Copy Encoder($x^{r\rightarrow t}$ ,$m^{r\rightarrow t}$) \\
%		}
%		Temporal attention score $T_{r}$ ,output $y^{t1}$, left-over mask $m^{t1}$ = Temporal inpainting($F^t$ ,$F^r\rightarrow t$,$m^t$,$m^{r\rightarrow t}$) ($r$ in $i_{ref}$) \\
%		\If{r is t-1 or t-2 }{
%			Warp Resiudal $R^{r\rightarrow t}$ using $F^r_{trans}$ 
%		}
%		\Else{
%			Warp Resiudal $R^{r\rightarrow t}$ using $A^r_{trans}$ ($r$ in $i_{ref}$)   \\
%		}
%		Temporal residual $Res^t$ = Temporal Attention transfer ($R^{r\rightarrow t}$,$T_{r}$ ,$M^r$) ($r$ in $i_{ref}$)\\
%		Output $Y^{t}$ Upsample $y^{t1}$ and add $Res^t$ \\
%		Update $R^t$ with $Res^t$\\
%		Update $x^t$ with $y^{t1}$\\
%		\If{$m^{t1}$ has any non zero values}{
%			Output $y^{t2}$ , Spatial attention score $S_{i,j}$ = Spatial Aggregation Network($y^{t1}$ ,$m^{t1}$) \\
%			Spatial Residual $Res^s$ = Attention transfer ($S_{i,j}$ ,$R^t$ ) \\
%			Output $Y^{t}$ Upsample $y^{t2}$ and add $Res^s$ \\
%			Update $R^t$ with $Res^s$ \\
%			Update $x^t$ with $y^{t2}$\\
%		}
%		}
%	
%\end{algorithm}

==> supp_details.tex <==

\section{Loss Functions}
\rev{
The definition of loss functions are similar as in CPNet \cite{lee2019copy} and HiFill \cite{yi2020contextual}.
The main difference is how the output of the main steps is calculated, e.g., we use the joint alignment while CPNet only uses the affine alignment. Also, our multi-scale spatial aggregation only applies on the leftover mask region instead of the full mask as in HiFill.
Also, note that the loss functions are used to train the STA-Net which works on the downsampled low resolution frames.
The specific definitions are as follows:
\vspace{-10pt}
\begin{equation}
L_{align} = \frac{1}{N} \cdot {\sum_{t}^{N} \sum_{r}  \mid \mid (1-M^{t}) \odot (1-M^{r \rightarrow t}) \odot (X^{t} -X^{r \rightarrow t}) \mid \mid _1}
\label{eq:align}
\end{equation}

\vspace{-12pt}

\begin{equation}
L_{hole(visible)} = \frac{1}{N} \cdot {\sum_{t}^{N}  \mid \mid M^{t} \odot C_{visible} \odot (Y^{t} -Y_{GT}^{t} ) \mid \mid _1} 
\label{eq:vis}
\end{equation}

\vspace{-10pt}

\begin{equation}
L_{hole(leftover)} = \frac{1}{N} \cdot {\sum_{t}^{N} \mid \mid M_{leftover}^t \odot (Y^{t} -Y_{GT}^{t} ) \mid \mid _1
\label{eq:leftover}} 
\end{equation}

\vspace{-8pt}

\begin{equation}
L_{non-hole} = \frac{1}{N} \cdot {\sum_{t}^{N}  \mid \mid (1 - M^t )\odot (Y^{t} - Y_{GT}^{t} ) \mid \mid _1
\label{eq:non-hole}} 
\end{equation}

\vspace{-8pt}

\begin{equation}
L_{perceptual} = \frac{1}{N} \cdot {\sum_{t}^{N} \frac{1}{P} \cdot \sum_{p}^{P}  \mid \mid \phi_p(Y_{comb}^{t}) - \phi_p(Y_{GT}^{t})  \mid \mid _1} 
\label{eq:percep}
\end{equation}

\vspace{-8pt}

\begin{equation}
L_{style} = \frac{1}{N} \cdot {\sum_{t}^{N} \frac{1}{P} \cdot \sum_{p}^{P}  \mid \mid G^{\phi}_p(Y_{comb}^{t}) - G^{\phi}_p(Y_{GT}^{t})  \mid \mid _1} 
\label{eq:style}
\end{equation}

\vspace{-10pt}

\begin{equation}
L_{rec} = \frac{1}{N} \cdot {\sum_{t}^{N}  \mid \mid M_{leftover}^t \odot (\tilde{X}^t - X^t)  \mid \mid _1 
+  \mid \mid (1- M_{leftover}^t) \odot ( \tilde{X}^t - X^t) \mid \mid _1} 
\label{eq:rec}
\end{equation}

\vspace{-10pt}

\begin{equation}
L_{adv} = \frac{1}{N} \cdot {\sum_{t}^{N} -\mathbb{E}_{{\tilde{X}^t} \in \mathbb{P}_g}  [ D(\tilde{X}^t) ]}
\label{eq:adv}
\end{equation}

% \tilde{X}^t = G(X^t, M_{t})

% \begin{equation}
% L_{adv} = \mathbb{E}_{{Y^t} \in \mathbb{P}_g}  [ D(Y^t) ] - \mathbb{E}_{{Y_{GT}^t} \in \mathbb{P}_r}  [ D(Y_{GT}^t) ] + \lambda \mathbb{E}_{{Y^t} \in \mathbb{P}_g}  [ D(Y^t) ]
% \end{equation}

In above equations, $X^t$ is the downsampled input frame at time $t$ and $M^t$ is its corresponding input mask.
$Y^t$ is the final inpainting result of $X^t$ and $Y_{GT}^t$ is the ground truth for $Y^t$.
$N$ is the number of frames in each sample of the training videos.
For our current training data, $N=5$.
$\odot$ is the element-wise multiplication.
In Equation \ref{eq:align}, $X^{r \rightarrow t}$ and $M^{r \rightarrow t}$ is the aligned reference frame and its aligned mask computed by aligning the reference frame $X^r$ to $X^t$ using the joint alignment module.
In Equation \ref{eq:vis} and \ref{eq:leftover}, $C_{visible}$ is the aggregated temporal attention scores (see the main paper and \cite{lee2019copy} for the definition);
$M_{leftover}^t$ is the leftover mask for frame $t$ which is defined as $M_{leftover}^t = M^t \odot (1-C_{visible})$.
In Equation \ref{eq:percep} and \ref{eq:style}, $Y_{comb}^t$ is the combination of the inpainting output $Y^t$ in the hole region and the input $X^t$ outside the hole;
$p$ is the index of the pooling layer in VGG-16 \cite{Simonyan15_vgg} and $\phi_p(\cdot)$ is the output of the corresponding layer;
$G_p^{\phi}(\cdot)$ is the gram matrix
multiplication \cite{johnson2016perceptual}.
In Equation \ref{eq:rec} and \ref{eq:adv}, $\tilde{X}^t$ is the generator output which is defined as $\tilde{X}^t = G(X^t, M_{leftover}^{t})$, where $G(\cdot, \cdot)$ is the generator;
$D(\cdot)$ is the discriminator and $\mathbb{P}_g$ is the distribution of the input frames. Note that the adversarial training loss is designed in the same way as in \cite{yi2020contextual}. More details about defining the WGAN-GP loss for the multi-scale spatial aggregation can also be found in \cite{yi2020contextual}}


\section{More Training Details}
In this section, we provide more details about training the STA-Net. The network is trained
on the proposed synthetic training dataset which contains numerous short video clips and the
ground truth object masks. We train the model on 2 Tesla V100 GPUs for 10 epochs with
the batch size set to 40. 
In our experiments, we increase the weight of $L_{align}$ so that the alignment module gets trained first and the later training converges faster.
The joint alignment and temporal aggregation parts of the network
are warmed-up for 2 epochs before adding the spatial aggregation module to the network for
training stability reasons. The model is implemented in PyTorch.

%\paragraph{Spatial aggregation losses.}
%Our spatial aggregation network adopts the generator in contextual residual aggregation framework  \cite{yi2020contextual}, which is trained using WGAN-GP loss \cite{gulrajani2017improved}. It also uses a reconstruction loss as a weighted pixelwise L1 distance between generator output and ground truth images based on the mask, which forces the consistency of the prediction with the original image. 
%\qt{please add some description about the new things you have to do when you combine the temporal aggregation network together with the spatial aggregration network}

%\begin{algorithm}
%	\small
%	\caption{Inference}
%	\label{alg:inference}
%	\SetAlgoLined
%	Input: Raw frame $X^t$ with mask $M^t$ ($t = 0,1,...,n$) \\	
%	Input: Downsampled frame $x^t$ (bilinear) with mask $m^t$ (nearest) ($t = 0,1,...,n$) \\
%	Input: Upsample $x^t$ and substract from  $X^t$ to calcualte residuals $R^t$ ($t = 0,1,...,n$)\\
%	Input: Number of reference frame for $N_{ref}$\\
%	Output: Inpainted frame $Y^{t2}$ ($t = 0,1,...,n$) \\
%	\For{t = 1,2,...,T-1}{
%		calcuated indices for refernce frame $i_{ref}$ = ($t-N_{ref}$,...,$t+N_{ref}$) \\
%		Multi-scale Target Copy features $F^t$ = Copy Encoder($x^t$,$m^t$) \\
%		\For{r in $i_{ref}$}{
%			\If{r is t-1 or t-2 }{ 
%				Flow $F^r_{trans}$ = PWC-IRR ($x^t$,$x^r$) \\
%				$x^{r\rightarrow t}$ ,$m^{r\rightarrow t}$ = Warp ($x^r$,$m^t$,$F^r_{trans}$) \\
%			}
%			\Else{
%				Affine Transformation $A^r_{trans}$ = Alignment Network($x^t$,$m^t$ ,$x^r$,$m^t$) \\
%				$x^{r\rightarrow t}$ ,$m^{r\rightarrow t}$ = Warp ($x^r$,$m^t$,$A^r_{trans}$) \\
%			}
%		
%			
%			Multi-scale Reference Copy features $F^r\rightarrow t$ = Copy Encoder($x^{r\rightarrow t}$ ,$m^{r\rightarrow t}$) \\
%		}
%		Temporal attention score $T_{r}$ ,output $y^{t1}$, left-over mask $m^{t1}$ = Temporal inpainting($F^t$ ,$F^r\rightarrow t$,$m^t$,$m^{r\rightarrow t}$) ($r$ in $i_{ref}$) \\
%		\If{r is t-1 or t-2 }{
%			Warp Resiudal $R^{r\rightarrow t}$ using $F^r_{trans}$ 
%		}
%		\Else{
%			Warp Resiudal $R^{r\rightarrow t}$ using $A^r_{trans}$ ($r$ in $i_{ref}$)   \\
%		}
%		Temporal residual $Res^t$ = Temporal Attention transfer ($R^{r\rightarrow t}$,$T_{r}$ ,$M^r$) ($r$ in $i_{ref}$)\\
%		Output $Y^{t}$ Upsample $y^{t1}$ and add $Res^t$ \\
%		Update $R^t$ with $Res^t$\\
%		Update $x^t$ with $y^{t1}$\\
%		\If{$m^{t1}$ has any non zero values}{
%			Output $y^{t2}$ , Spatial attention score $S_{i,j}$ = Spatial Aggregation Network($y^{t1}$ ,$m^{t1}$) \\
%			Spatial Residual $Res^s$ = Attention transfer ($S_{i,j}$ ,$R^t$ ) \\
%			Output $Y^{t}$ Upsample $y^{t2}$ and add $Res^s$ \\
%			Update $R^t$ with $Res^s$ \\
%			Update $x^t$ with $y^{t2}$\\
%		}
%		}
%	
%\end{algorithm}




==> supp_results.tex <==

\section{More Experiment Results}
\paragraph{Qualitative comparison.}
In Figure \ref{fig:compare_vin} and \ref{fig:compare_syn}, we show more results for qualitative comparisons of our methods with the state-of-the-art learning and flow-based methods on the
synthetic $\text{Syn-DS}^{+}$ and real world HIN dataset. We also attach a demo video that compares
results from different methods for video inpainting on 1080p videos from the $\text{DS}^{+}$ \cite{Perazzi2016} and
the HIN dataset.
Note that some baselines cannot directly run on 1080p videos due to memory constraint.
Therefore, we run these baselines on 1792x960 resolution and then resize the output to 1080p.
The improvements of our method upon others can be observed more clearly
in the video. The results show that the learning based method STTN \cite{zeng2020learning} tends to generate
blurry inpaintings and the flow-based method FGVC \cite{gao2020flow} may produce artifacts near the mask
boundaries. Our results are more temporally coherent and visually appealing.

   \begin{figure} [t]
	\centering
	\includegraphics[width=0.98\linewidth]{figs/compare_syn.pdf}
	\vspace{-10pt}
	\caption{Video inpainting results on $\text{Syn-DS}^{+}$ dataset: (a) Input frame with mask (1728x960)
(b) STTN (c) FGVC (d) Ours (e) Ground Truth.}
	\label{fig:compare_syn}
	\vspace{-5pt}
\end{figure}

  \begin{figure} [!t]
 	\centering
 	\includegraphics[width=0.85\linewidth]{figs/user_study_small.pdf}
 	\vspace{-10pt}
 	\caption{User study on 30 tasks composed of videos from $\text{DS}^{+}$ and HIN. “Rank x” means
the percentage of results from each model being chosen as the x-th best.}
 	\label{fig:user_study}
 	\vspace{-5pt}
 \end{figure}


 
%   \begin{figure*}[t]
%  	\centering
%  	\includegraphics[width=0.95\linewidth]{temporal_ablation_supp.pdf}
%  	\vspace{-10pt}
%  	\caption{Ablation study for temporal modules on HIN: (a) Input frame with mask (270p) (b) Vanila temporal aggregation (270p) (c) Multi-scale temporal aggregation (270p) (d) After bilinear upsampling (1080p) (e) With temporal residuals add to (d). }
%  	\label{fig:temp_ablation}
%  	\vspace{-5pt}
%  \end{figure*}

\paragraph{User Study.}
In the user study, there are 30 tasks composed of video inpainting results generated at 1728x960 resolution of
the $\text{DS}^{+}$ and HIN dataset . In each task, the input video with the masks is first shown to the user, then results of the four methods are randomly arranged. The user is asked to rank
the four results based on two criteria: 1) whether the inpainted videos look like real; 2)
whether the inpainting results are spatially and temporally consistent. Figure \ref{fig:user_study} summarizes
the user study results. It can be found that our results are comparable to the state-of-theart flow-based method FGVC while outperform the learning-based methods CPNet \cite{lee2019copy} and
STTN comfortably for the high resolution videos. Another important observation is our method has
the lowest percentage of being ranked as the last which shows the robustness of our method.



% \subsection{Ablation Studies.}
% \paragraph{Qualitative ablation study on the temporal modules.}
% In Figure \ref{fig:temp_ablation}, we show additional
% results for evaluating the contribution of different temporal modules on the HIN dataset.
 

% \paragraph{Qualitative ablation study on the spatial aggregation module.}
% We show the result of the
% qualitative ablation study on the spatial aggregation in Figure \ref{fig:spatial_aggregation}. Here, we can see the contribution of our multi-scale spatial aggregation network for improving the inpainting quality on
% the central regions where no information has been transferred from other temporal reference
% frames, e.g., the region covered by the leftover mask.
%by borrowing patches from spatial context for the region covered by the leftover mask.

% \paragraph{Quantitative ablation study on the alignment method.}
%  In Table \ref{table:alignment_abl}, quantitative results verify that our combined alignment method can generally improve the performance of each individual method.
 


%  \begin{table}[t]
%  	\centering
%  	\addtolength{\tabcolsep}{-3pt}
%  	\begin{tabular}{l | ccc }
%  		%		&  \multicolumn{3}{c}{Metrics} \\
%  		%		\hline
%  		\multicolumn{1}{c|}{Alignment Method}  &   L1 $\downarrow$  &   SSIM $\uparrow$  & PSNR $\uparrow$ \\
%  		\hline
%  		%		\hline
%  		Affine transformation & 0.005 & \textbf{0.98} & 32.05\\
%  		Optical flow  & 0.017 & 0.927 & 29.21 \\
%  		Both  & \textbf{0.003} & 0.97 & \textbf{33.14} \\		
%  	\end{tabular}
%  	\caption{Quantitative ablation study for different image alignment methods on the $\text{Syn-DS}^{+}$
% dataset. Results are generated at 1080p resolution.}
%  	\label{table:alignment_abl}
%  \end{table}
 


 

 
 

